What you see is (not) what you get: A VR Framework for Correcting Robot Errors

Many solutions tailored for intuitive visualization or teleoperation of virtual, augmented and mixed (VAM) reality systems are not robust to robot failures, such as the inability to detect and recognize objects in the environment or planning unsafe trajectories. In this paper, we present a novel virtual reality (VR) framework where users can (i) recognize when the robot has failed to detect a real-world object, (ii) correct the error in VR, (iii) modify proposed object trajectories and, (iv) implement behaviors on a real-world robot. Finally, we propose a user study aimed at testing the efficacy of our framework. Project materials can be found in the OSF repository.

==> figures/ds.tex <==
\begin{tikzpicture}[auto,node distance=1cm and 1cm,on grid]%
    % Define block styles
    % \tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    %     text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
    \tikzstyle{scenario} = [rectangle, draw, fill=green!10, 
        text width=6em, text centered, minimum height=3em]
    \tikzstyle{map} = [rectangle, draw, fill=orange!10, 
        text width=9em, text centered, rounded corners, minimum height=2em]
    \tikzstyle{line} = [draw]
    \tikzstyle{element} = [ellipse, draw, fill=blue!10, 
        text width=4.2em, text centered, minimum height=2em]
    \tikzstyle{other} = [rectangle, draw, fill=red!10, 
        text width=7em, text centered, rounded corners, minimum height=2em]
    % \tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    %     minimum height=2em]
    
    \newcommand*{\connectorH}[4][]{
        \draw[#1] (#3) -| ($(#3) !#2! (#4)$) |- (#4)
    }
    \newcommand*{\connectorV}[4][]{
        \draw[#1] (#3) |- ($(#3) !#2! (#4)$) -| (#4)
    }
    \newcommand*{\connectorHLast}[4][4]{
        \draw[#1] let
                \p1 = (#3),
                \p2 = ($(#3) !#2! (#4)$)
            in (\x2,\y1) |- (#4)
    }
    \newcommand*{\connectorVLast}[4][4]{
        \draw[#1] let
                \p1 = (#3),
                \p2 = ($(#3) !#2! (#4)$)
            in (\x1,\y2) -| (#4)
    }

    % Place nodes
    \node [scenario] (autonomous_driving_maps) {Autonomous Driving Maps};
    
    \node [map, above right=1.5cm and 4cm of autonomous_driving_maps] (hd_maps) {HD maps};
    \node [map, above right=0.5cm and 4cm of autonomous_driving_maps] (feature_based) {Feature maps};
    \node [map, below right=0.5cm and 4cm of autonomous_driving_maps] (grid_maps) {Grid maps};
    \node [map, below right=1.5cm and 4cm of autonomous_driving_maps] (dense_point_cloud) {Dense point cloud};
    
    % \node [element, above right=5mm and 3cm of hd_maps] (vector_map) {Lanelets};
    % \node [element, below right=5mm and 3cm of hd_maps] (rasterized) {Rasterized};

    % \node [element, right=3cm of grid_maps] (elevation) {Elevation};
    % \node [element, above right=10mm and 3cm of grid_maps] (cells) {Cells};
    % \node [element, below right=10mm and 3cm of grid_maps] (voxels) {Voxels};
    
    % Draw edges
    \connectorH [line] {0.50}{autonomous_driving_maps.east}{feature_based.west};
    \connectorHLast [line] {0.50}{autonomous_driving_maps.east}{grid_maps.west};
    % Ensure that two lines do not overlap (just to make it look a bit nicer in PDF viewers with bad AA)
    \path [line] let
            \p1 = ($(autonomous_driving_maps.east) !0.5! (feature_based.west)$),
            \p2 = (feature_based.west)
        in (\x1,\y2) |- (hd_maps.west);
    \path [line] let
            \p1 = ($(autonomous_driving_maps.east) !0.5! (grid_maps.west)$),
            \p2 = (grid_maps.west)
        in (\x1,\y2) |- (dense_point_cloud.west);
    
    % \connectorH [line] {0.50}{hd_maps.east}{vector_map.west};
    % \connectorHLast [line] {0.50}{hd_maps.east}{rasterized.west};
    
    % \connectorHLast [line] {0.50}{grid_maps.east}{cells.west};
    % \path [line] (grid_maps.east) -- (elevation.west);
    % \connectorHLast [line] {0.50}{grid_maps.east}{voxels.west};
\end{tikzpicture}%

==> figures/ds_old.tex <==
\begin{tikzpicture}[auto,node distance=1.5cm]
    % Define block styles
    % \tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    %     text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
    \tikzstyle{scenario} = [rectangle, draw, fill=green!10, 
        text width=6em, text centered, minimum height=3em]
    \tikzstyle{map} = [rectangle, draw, fill=orange!10, 
        text width=7em, text centered, rounded corners, minimum height=2em]
    \tikzstyle{line} = [draw]
    \tikzstyle{element} = [ellipse, draw, fill=blue!10, 
        text width=4.2em, text centered, minimum height=2em]
    \tikzstyle{other} = [rectangle, draw, fill=red!10, 
        text width=7em, text centered, rounded corners, minimum height=2em]
    % \tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    %     minimum height=2em]
    
    \newcommand*{\connectorH}[4][]{
        \draw[#1] (#3) -| ($(#3) !#2! (#4)$) |- (#4)
    }
    \newcommand*{\connectorV}[4][]{
        \draw[#1] (#3) |- ($(#3) !#2! (#4)$) -| (#4)
    }
    \newcommand*{\connectorHLast}[4][4]{
        \draw[#1] let
                \p1 = (#3),
                \p2 = ($(#3) !#2! (#4)$)
            in (\x2,\y1) |- (#4)
    }
    \newcommand*{\connectorVLast}[4][4]{
        \draw[#1] let
                \p1 = (#3),
                \p2 = ($(#3) !#2! (#4)$)
            in (\x1,\y2) -| (#4)
    }

    % Place nodes
    \node [scenario] (autonomous_driving_maps) {Autonomous Driving Maps};
    
    \node [map, right=2cm of autonomous_driving_maps] (grid_maps) {Grid maps};
    \node [map, above right=1.5cm and 1cm of autonomous_driving_maps] (vector_maps) {Vector maps};
    \node [map, below right=1.5cm and 1cm of autonomous_driving_maps] (other_solutions) {Other solutions};

    \node [element, right=4cm of grid_maps] (voxels) {Voxels};
    \node [element, above=2mm of voxels] (cells) {Cells};
    \node [element, below=2mm of voxels] (stixels) {Stixels};
    
    \node [element, above right=0mm and 2cm of vector_maps] (lanelet) {Lanelet};
    \node [element, below right=0mm and 2cm of vector_maps] (raserized) {Rasterized};
    
    \node [other, above right=0mm and 2cm of other_solutions] (feature_based) {Feature based};
    \node [other, below right=0mm and 2cm of other_solutions] (dense_point_cloud) {Dense point cloud};
    
    % Draw edges
    \path [line] (autonomous_driving_maps.east) -- (grid_maps.west);
    \connectorHLast [line] {0.50}{autonomous_driving_maps.east}{vector_maps.west};
    \connectorHLast [line] {0.50}{autonomous_driving_maps.east}{other_solutions.west};
    
    \path [line] (grid_maps.east) -- (voxels.west);
    \connectorHLast [line] {0.50}{grid_maps.east}{cells.west};
    \connectorHLast [line] {0.50}{grid_maps.east}{stixels.west};
    
    \connectorH [line] {0.50}{vector_maps.east}{lanelet.west};
    \connectorHLast [line] {0.50}{vector_maps.east}{raserized.west};
    
    \connectorH [line] {0.50}{other_solutions.east}{feature_based.west};
    \connectorHLast [line] {0.50}{other_solutions.east}{dense_point_cloud.west};
\end{tikzpicture}%

==> figures/ds_prev.tex <==
\begin{tikzpicture}[auto,node distance=1cm and 1cm,on grid]%
    % Define block styles
    % \tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    %     text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
    \tikzstyle{scenario} = [rectangle, draw, fill=green!10, 
        text width=6em, text centered, minimum height=3em]
    \tikzstyle{map} = [rectangle, draw, fill=orange!10, 
        text width=7em, text centered, rounded corners, minimum height=2em]
    \tikzstyle{line} = [draw]
    \tikzstyle{element} = [ellipse, draw, fill=blue!10, 
        text width=4.2em, text centered, minimum height=2em]
    \tikzstyle{other} = [rectangle, draw, fill=red!10, 
        text width=7em, text centered, rounded corners, minimum height=2em]
    % \tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    %     minimum height=2em]
    
    \newcommand*{\connectorH}[4][]{
        \draw[#1] (#3) -| ($(#3) !#2! (#4)$) |- (#4)
    }
    \newcommand*{\connectorV}[4][]{
        \draw[#1] (#3) |- ($(#3) !#2! (#4)$) -| (#4)
    }
    \newcommand*{\connectorHLast}[4][4]{
        \draw[#1] let
                \p1 = (#3),
                \p2 = ($(#3) !#2! (#4)$)
            in (\x2,\y1) |- (#4)
    }
    \newcommand*{\connectorVLast}[4][4]{
        \draw[#1] let
                \p1 = (#3),
                \p2 = ($(#3) !#2! (#4)$)
            in (\x1,\y2) -| (#4)
    }

    % Place nodes
    \node [scenario] (autonomous_driving_maps) {Autonomous Driving Maps};
    
    \node [map, above right=2.0cm and 3.5cm of autonomous_driving_maps] (hd_maps) {HD maps};
    \node [map, above right=0.7cm and 3.5cm of autonomous_driving_maps] (feature_based) {Feature based};
    \node [map, below right=0.7cm and 3.5cm of autonomous_driving_maps] (grid_maps) {Grid maps};
    \node [map, below right=2.0cm and 3.5cm of autonomous_driving_maps] (dense_point_cloud) {Dense point cloud};
    
    \node [element, above right=5mm and 3.5cm of hd_maps] (vector_map) {Vector};
    \node [element, below right=5mm and 3.5cm of hd_maps] (rasterized) {Rasterized};

    \node [element, right=3.5cm of grid_maps] (elevation) {Elevation};
    \node [element, above right=10mm and 3.5cm of grid_maps] (cells) {Cells};
    \node [element, below right=10mm and 3.5cm of grid_maps] (voxels) {Voxels};
    
    % Draw edges
    \connectorH [line] {0.50}{autonomous_driving_maps.east}{feature_based.west};
    \connectorHLast [line] {0.50}{autonomous_driving_maps.east}{grid_maps.west};
    % Ensure that two lines do not overlap (just to make it look a bit nicer in PDF viewers with bad AA)
    \path [line] let
            \p1 = ($(autonomous_driving_maps.east) !0.5! (feature_based.west)$),
            \p2 = (feature_based.west)
        in (\x1,\y2) |- (hd_maps.west);
    \path [line] let
            \p1 = ($(autonomous_driving_maps.east) !0.5! (grid_maps.west)$),
            \p2 = (grid_maps.west)
        in (\x1,\y2) |- (dense_point_cloud.west);
    
    \connectorH [line] {0.50}{hd_maps.east}{vector_map.west};
    \connectorHLast [line] {0.50}{hd_maps.east}{rasterized.west};
    
    \connectorHLast [line] {0.50}{grid_maps.east}{cells.west};
    \path [line] (grid_maps.east) -- (elevation.west);
    \connectorHLast [line] {0.50}{grid_maps.east}{voxels.west};
\end{tikzpicture}%
